Bilateral Self-unbiased Learning from Biased Implicit Feedback

Implicit feedback has been widely used to build commercial recommender systems. Because observed feedback represents users' click logs, there is a semantic gap between true relevance and observed feedback. More importantly, observed feedback is usually biased towards popular items, thereby overestimating the actual relevance of popular items. Although existing studies have developed unbiased learning methods using inverse propensity weighting (IPW) or causal reasoning, they solely focus on eliminating the popularity bias of items. In this paper, we propose a novel unbiased recommender learning model, namely BIlateral SElf-unbiased Recommender (BISER), to eliminate the exposure bias of items caused by recommender models. Specifically, BISER consists of two key components: (i) self-inverse propensity weighting (SIPW) to gradually mitigate the bias of items without incurring high computational costs; and (ii) bilateral unbiased learning (BU) to bridge the gap between two complementary models in model predictions, i.e., user- and item-based autoencoders, alleviating the high variance of SIPW. Extensive experiments show that BISER consistently outperforms state-of-the-art unbiased recommender models over several datasets, including Coat, Yahoo! R3, MovieLens, and CiteULike.

==> Figures/exp-fig-mf_self.tex <==
\begin{figure}[t!]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.21\textwidth]{Figures/graph_mf_ml-100k_prediction_matrix_top50_onlymissing.csv.png} &
\includegraphics[width=0.21\textwidth]{Figures/graph_crmf_self_ml-100k_prediction_matrix_top50_onlymissing.csv.png} \\
\multicolumn{1}{c}{(a) MF} &\multicolumn{1}{c}{(b) Unbiased MF (ours)}
% \vspace{4mm}
\end{tabular}
\caption{Item distributions for MF and our Unbiased MF on ML-100K. All items are top-50 recommended items for each user. The y-axis means that the sorted item id by item popularity. That is, the larger the item id, the more popular it is. While MF mainly recommends popular items, the unbiased MF recommends more diverse items.}\label{fig:mf_self}
%\vskip -1.5
\end{figure}

==> Figures/exp-fig-ml100k.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{Figures/mar_legend.png}
\begin{tabular}{cc}
\includegraphics[width=0.22\textwidth]{Figures/ml100k_ndcg_50.csv.png} &
\includegraphics[width=0.22\textwidth]{Figures/ml100k_map_50.csv.png} \\
\vspace{-1mm}
\end{tabular}
\caption{Accuracy comparison with unbiased evaluation. The results are averaged over 5 runs on ML-100K. We also observe similar trends with other metrics, $@10$ and $@30$.}\label{fig:unbiased_eval_ml100k} 
% \end{figure*}

 %The similar trends are observed the results in the other metrics as well as results in NDCG$@$50 and MAP$@$50.

\vspace{6mm}

% \begin{figure*}[t]
\centering
\includegraphics[width=0.4\textwidth]{Figures/mar_legend.png}
\begin{tabular}{cccc}
\includegraphics[width=0.22\textwidth]{Figures/ml100k_ndcg_aoa_50.csv.png} &
\includegraphics[width=0.22\textwidth]{Figures/ml100k_map_aoa_50.csv.png} \\
\vspace{-1mm}
\end{tabular}
\caption{Accuracy comparison with AOA evaluation. The results are averaged over 5 runs on ML-100K. We also observe similar trends with other metrics, $@10$ and $@30$.}\label{fig:aoa_eval_ml100k}
\vspace{-1mm}
\end{figure}

==> Figures/exp-fig.tex <==
% \begin{figure}[t]
% \centering
% \begin{tabular}{cc}
% \includegraphics[width=0.22\textwidth]{Figures/ml100k_ndcg_10_unbiased_aoa_v3.png} &
% \includegraphics[width=0.22\textwidth]{Figures/ml100k_map_10_unbiased_aoa_v2.png} \\
% \end{tabular}
% \vspace{-4mm}
% \caption{Comparison of each model with AOA/unbiased evaluation on ML-100K.}\label{fig:cm100k}
% \vspace{-4mm}
% \end{figure}

\begin{figure}[t]
\centering
\vspace{-2mm}
\begin{tabular}{c}
% \includegraphics[width=0.47\textwidth]{Figures/ml100k_ndcg_10_unbiased_aoa_v3.png}
\includegraphics[width=0.42\textwidth]{Figures/ml100k_map_10_unbiased_aoa_v2.png}
\end{tabular}
\vspace{-4mm}
\caption{Comparison results with AOA and unbiased evaluation on ML-100K.}\label{fig:comparison_ml100k}
\vspace{-2mm}
\end{figure}


==> Tables/exe_table_ml100k_citeulike.tex <==
\begin{table*}[t]
\centering
\caption{Performances comparison of each model on Coat and Yahoo! R3 (the best in bold font, * and ** indicate $p < 0.005$ and $p < 0.001$ for an one-tailed t-test, $\dagger$ indicates the best baseline model for t-test and performance gain). The results are averaged over 10 and 5 runs on Coat and Yahoo! R3, respectively. Gain indicates an improvement ratio to the best baseline model.}\label{tab:ml100k_citeulike}
\begin{center}
\renewcommand{\arraystretch}{1.0} % 테이블 행 간격
\begin{tabular}{P{1.5cm}P{1.8cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}}
\toprule

\multicolumn{2}{c}{} & \multicolumn{3}{c}{NDCG$@N$} & \multicolumn{3}{c}{MAP$@N$} & \multicolumn{3}{c}{Recall$@N$}\\
\cmidrule(r){3-5}
\cmidrule(lr){6-8}
\cmidrule(l){9-11}
 Datasets & Models & $N$ = 1 & $N$ = 3 & $N$ = 5 & $N$ = 1 & $N$ = 3 & $N$ = 5 & $N$ = 1 & $N$ = 3 & $N$ = 5  \\
\hline
\multirow{8}{*}{ML-100K}
& MF        & 0.0148 & 0.0231 & 0.0274 & 0.0293 & 0.0402 & 0.0448 & 0.0707 & 0.1628 & 0.2281  \\
& UAE       & 0.0195 & 0.0283 & 0.0329 & 0.0391 & 0.0521 & 0.0575 & 0.0867 & 0.1884 & 0.2571  \\
& IAE       & 0.0192 & 0.0280 & 0.0322 & 0.0386 & 0.0515 & 0.0568 & 0.0861 & 0.1856 & 0.2513  \\
\cline{2-11}
& RelMF    & 0.0204 & 0.0309 & 0.0364 & 0.0411 & 0.0563 & 0.0629 & 0.0985 & 0.2231 & 0.3083  \\
& AT        & 0.0210 & 0.0314 & 0.0374 & 0.0426 & 0.0584 & 0.0658 & 0.1013 & 0.2244 & 0.3168  \\
& CJMF$^{\dagger}$      & 0.0211 & 0.0324 & 0.0382 & 0.0424 & 0.0591 & 0.0658 & 0.0974 & 0.2248 & 0.3126  \\
\cline{2-11}
& BISER (ours)  & 0.0217 & 0.0328 & 0.0386 & 0.0436 & 0.0594 & 0.0659 & 0.0963 & 0.2210 & 0.3077  \\

\cline{2-11}
& BISER (ours) & \textbf{0.4503}$^{*}$ & \textbf{0.4109}$^{*}$ & \textbf{0.4378}$^{**}$ & \textbf{0.1725}$^{*}$ & \textbf{0.2663}$^{**}$ & \textbf{0.3192}$^{**}$ & \textbf{0.1725}$^{*}$ & \textbf{0.3185}$^{*}$ & \textbf{0.4367}$^{**}$ \\
\cline{2-11}
& Gain (\%) & 10.03 & 6.56 & 6.85 & 14.99 & 10.58 & 10.08 & 14.99 & 6.74 & 7.16 \\
\hline
\multirow{8}{*}{CiteULike}
& MF & 0.1797 & 0.2081 & 0.2411 & 0.1071 & 0.1688 & 0.1970 & 0.1071 & 0.2225 & 0.3040 \\
& UAE & 0.1983 & 0.2235 & 0.2532 & 0.1198 & 0.1836 & 0.2104 & 0.1198 & 0.2362 & 0.3111 \\
& IAE & 0.2137 & 0.2355 & 0.2653 & 0.1309 & 0.1956 & 0.2232 & 0.1309 & 0.2461 & 0.3211 \\
\cline{2-11}
& RelMF & 0.1837 & 0.2122 & 0.2453 & 0.1102 & 0.1728 & 0.2014 & 0.1102 & 0.2266 & 0.3080 \\
& AT & 0.1912 & 0.2179 & 0.2506 & 0.1149 & 0.1786 & 0.2071 & 0.1149 & 0.2310 & 0.3125 \\
& CJMF$^{\dagger}$ & 0.2151 & 0.2426 & 0.2715 & 0.1320 & 0.2018 & 0.2291 & 0.1320 & 0.2564 & 0.3297 \\
\cline{2-11}
& BISER (ours) & \textbf{0.2323}$^{**}$ & \textbf{0.2608}$^{**}$ & \textbf{0.2894}$^{**}$ & \textbf{0.1446}$^{**}$ & \textbf{0.2195}$^{**}$ & \textbf{0.2479}$^{**}$ & \textbf{0.1446}$^{**}$ & \textbf{0.2748}$^{**}$ & \textbf{0.3477}$^{**}$ \\
\cline{2-11}
& Gain (\%) & 7.99 & 7.52 & 6.60 & 9.58 & 8.77 & 8.20 & 9.58 & 7.18 & 5.47 \\
 
\bottomrule
\end{tabular}
\end{center}
\end{table*}

==> Tables/exp_ablation.tex <==
% \begin{table}[t]
% \centering
% \caption{Comparison between MF against MF with propensity weights for unclicked feedback in two datasets.}\label{tab:negative_effect}
% \vspace{-3mm}

% \begin{center}
% \renewcommand{\arraystretch}{0.9} % 테이블 행 간격
% \begin{tabular}{P{1.1cm} P{2.5cm} P{1.2cm} P{1.1cm} P{1.1cm}}

% \toprule
%  Datasets & Models & MAP@1 & MAP@3 & MAP@5 \\
% \hline
% \multirow{3}{*}{Coat}
% & MF & 0.1346 & 0.2100 & 0.2566\\
% & \begin{tabular}{l}MF w/ propensity\\[-1pt] for unclicked bias\end{tabular} & \textbf{0.1440} & \textbf{0.2197} & \textbf{0.2633}\\
% \hline
% \multirow{3}{*}{Yahoo! R3}
% & MF & 0.1071 & 0.1688 & 0.1970 \\
% & \begin{tabular}{l}MF w/ propensity\\[-1pt] for unclicked bias\end{tabular} & \textbf{0.1351} & \textbf{0.2091} & \textbf{0.2380} \\
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table}

\begin{table}[t]
\centering
% \caption{Comparison of MF vs. MF w/ only unclicked propensity (\ie, neg. only) vs. MF w/ only clicked propensity (\ie, pos. only) in two benchmark datasets.}\label{tab:negative_effect}
\caption{Comparison of MF vs. MF w/ propensity weight for unclicked data (\ie, MF w/ neg.) on Coat and Yahoo! R3.}\label{tab:negative_effect}
\vspace{-3mm}

\begin{center}
\renewcommand{\arraystretch}{0.9} % 테이블 행 간격
\begin{tabular}{P{1.5cm} P{1.6cm} P{1.2cm} P{1.2cm} P{1.2cm}}

\toprule
 Datasets & Models & MAP@1 & MAP@3 & MAP@5 \\
\hline
\multirow{2}{*}{Coat}
& MF & 0.1346 & 0.2100 & 0.2566\\
& MF w/ neg. & \textbf{0.1492} & \textbf{0.2287} & \textbf{0.2746}\\
% & w/ neg. only & 0.1492 & 0.2287 & 0.2746\\
% & w/ pos. only & \textbf{0.1544} & \textbf{0.2324} & \textbf{0.2776}\\
% & MF-DU & 0.1566 & 0.2354 & 0.2821\\ %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline
\multirow{2}{*}{Yahoo! R3}
& MF & 0.1071 & 0.1688 & 0.1970 \\
& MF w/ neg. & \textbf{0.1277} & \textbf{0.1978} & \textbf{0.2271}\\
% & w/ neg. only & 0.1277 & 0.1978 & 0.2271\\
% & w/ pos. only & \textbf{0.1308} & \textbf{0.2028} & \textbf{0.2320} \\
% & MF-DU & 0.1373 & 0.2068 & 0.2364\\ %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> Tables/exp_hyperparameters.tex <==
\begin{table*}[h!]
\centering
\caption{The best hyperparameters in the five datasets, Coat, Yahoo! R3, ML-100K, ML-1M, and CiteULike.}\label{tab:hyperparameters}
\begin{center}
\renewcommand{\arraystretch}{1.0} % 테이블 행 간격
\begin{tabular}{P{1.4cm}P{2.6cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}}
\toprule
\multicolumn{2}{c}{} & \multicolumn{6}{c}{Models} \\
\cmidrule(l){3-8}
Datasets & Hyperparameters & UAE~\cite{SedhainMSX15} & IAE~\cite{SedhainMSX15} & MF~\cite{HuKV08} & RelMF~\cite{SaitoYNSN20} & AT~\cite{Saito20at} & CJMF~\cite{ZhuHZC20} \\

\hline
\multirow{4}{*}{Coat}
 & Learning rate    & 0.1      & 0.2    & 0.005    & 0.005    & 0.0005  & 0.005    \\
 & Regularization   & 1E-06    & 1E-07  & 1E-09    & 1E-05    & 1E-10   & 1E-09    \\
 & Latent dimension & 50       & 50     & 128      & 128      & 128     & 128      \\
 & Batch size       & 1        & 1      & 1024     & 1024     & 1024    & 1024     \\
\hline
\multirow{4}{*}{Yahoo! R3}
 & Learning rate    & 0.01     & 0.05   & 0.001    & 0.001    & 0.0001  & 0.001    \\
 & Regularization   & 0        & 0      & 1E-07    & 1E-07    & 1E-14   & 1E-06    \\
 & Latent dimension & 200      & 200    & 64       & 64       & 64      & 64       \\
 & Batch size       & 1        & 1      & 1024     & 1024     & 1024    & 1024     \\
\hline
\multirow{4}{*}{ML-100K}
 & Learning rate    & 0.01     & 0.01   & 0.001    & 0.001    & 0.0001  & 0.001    \\
 & Regularization   & 1E-04    & 1E-04  & 1E-06    & 1E-06    & 1E-10   & 1E-09    \\
 & Latent dimension & 200      & 200    & 64       & 64       & 64      & 64       \\
 & Batch size       & 1        & 1      & 1024     & 1024     & 1024    & 1024     \\
\hline
\multirow{4}{*}{ML-1M}
 & Learning rate    & 0.01     & 0.01   & 0.0005   & 0.0005   & 0.00005 & 0.001    \\
 & Regularization   & 0        & 0      & 1E-08    & 1E-07    & 1E-9    & 0        \\
 & Latent dimension & 200      & 200    & 64       & 64       & 64      & 128      \\
 & Batch size       & 1        & 1      & 1024     & 1024     & 1024    & 1024     \\
\hline
\multirow{4}{*}{CiteULike}
 & Learning rate    & 0.2      & 0.1    & 0.001    & 0.0005   & 0.00005 & 0.005    \\
 & Regularization   & 0        & 0      & 1E-09    & 1E-09    & 1E-09   & 1E-13    \\
 & Latent dimension & 200      & 200    & 128      & 128      & 128     & 128      \\
 & Batch size       & 1        & 1      & 16384    & 16384    & 16384   & 16384    \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

% 나머지 hyperparameter 설명
% The cliping values ($\mu, \nu$) in Rel-MF, DualUMF are all 0.1. Also, In ExpoMF, all of hyperparameter except the hidden dimension are used as default values in the given code ($\lambda_{\theta}, \lambda_{\beta}, \lambda_{y}, \mu_{ui}$ are 1e-5, 1e-5, 1.0, 0.01).

==> Tables/exp_table_cu_1.tex <==
\begin{table*}[t]
\centering
\caption{Effects of complementary unbiased learning of each model on two benchmark datasets.}\label{tab:cu1}
\begin{center}
\begin{tabular}{P{1.5cm}P{2.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}}
\toprule

\multicolumn{2}{c}{} & \multicolumn{3}{c}{NDCG@K} & \multicolumn{3}{c}{MAP@K} & \multicolumn{3}{c}{Recall@K}\\
\cmidrule(r){3-5}
\cmidrule(lr){6-8}
\cmidrule(l){9-11}
 Datasets & Models & K = 1 & K = 3 & K = 5 & K = 1 & K = 3 & K = 5 & K = 1 & K = 3 & K = 5  \\
\hline
\multirow{8}{*}{Coat}
& uAE & 0.3610 & 0.3546 & 0.3815 & 0.1265 & 0.2165 & 0.2648 & 0.1265 & 0.2785 & 0.3869 \\
& uAE w/ CU & 0.3624 & 0.3584 & 0.3822 & 0.1257 & 0.2176 & 0.2644 & 0.1257 & 0.2834 & 0.3885 \\
& uAE w/ SU & 0.4262 & 0.3973 & 0.4259 & 0.1623 & 0.2538 & 0.3063 & 0.1623 & 0.3100 & 0.4302 \\
& uAE w/ SU, CU & 0.4321 & 0.4021 & 0.4322 & 0.1651 & 0.2589 & 0.3126 & 0.1651 & 0.3152 & 0.4388 \\
\cline{2-11}
& iAE & 0.3655 & 0.3560 & 0.3812 & 0.1311 & 0.2185 & 0.2651 & 0.1311 & 0.2769 & 0.3847 \\
& iAE w/ CU & 0.3709 & 0.3611 & 0.3866 & 0.1316 & 0.2218 & 0.2691 & 0.1316 & 0.2835 & 0.3921 \\
& iAE w/ SU & 0.4334 & 0.3949 & 0.4172 & 0.1650 & 0.2529 & 0.3007 & 0.1650 & 0.3024 & 0.4120 \\
& iAE w/ SU, CU & 0.4322 & 0.3986 & 0.4242 & 0.1654 & 0.2562 & 0.3067 & 0.1654 & 0.3084 & 0.4234 \\
\hline
\multirow{8}{*}{Yahoo}
& uAE &  &  &  &  &  &  &  &  &  \\
& uAE w/ CU &  &  &  &  &  &  &  &  &  \\
& uAE w/ SU &  &  &  &  &  &  &  &  &  \\
& uAE w/ SU, CU &  &  &  &  &  &  &  &  &  \\
\cline{2-11}
& iAE &  &  &  &  &  &  &  &  &  \\
& iAE w/ CU &  &  &  &  &  &  &  &  &  \\
& iAE w/ SU &  &  &  &  &  &  &  &  &  \\
& iAE w/ SU, CU &  &  &  &  &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> Tables/exp_table_cu_2.tex <==
\begin{table*}[t]
\centering
\caption{Performance comparison of each model on two benchmark datasets.}\label{tab:cu2}
\begin{center}
\begin{tabular}{P{1.5cm}P{1.5cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}}
\toprule

\multicolumn{2}{c}{} & \multicolumn{3}{c}{NDCG@K} & \multicolumn{3}{c}{MAP@K} & \multicolumn{3}{c}{Recall@K}\\
\cmidrule(r){3-5}
\cmidrule(lr){6-8}
\cmidrule(l){9-11}
 Datasets & Models & K = 1 & K = 3 & K = 5 & K = 1 & K = 3 & K = 5 & K = 1 & K = 3 & K = 5  \\
\hline
\multirow{4}{*}{Coat}
& uAE & 0.3610 & 0.3546 & 0.3815 & 0.1265 & 0.2165 & 0.2648 & 0.1265 & 0.2785 & 0.3869 \\
& uAE w/ CU & 0.3624 & 0.3584 & 0.3822 & 0.1257 & 0.2176 & 0.2644 & 0.1257 & 0.2834 & 0.3885 \\
\cline{2-11}
& iAE & 0.3655 & 0.3560 & 0.3812 & 0.1311 & 0.2185 & 0.2651 & 0.1311 & 0.2769 & 0.3847 \\
& iAE w/ CU & 0.3709 & 0.3611 & 0.3866 & 0.1316 & 0.2218 & 0.2691 & 0.1316 & 0.2835 & 0.3921 \\
\hline
\multirow{4}{*}{Yahoo}
& uAE &  &  &  &  &  &  &  &  &  \\
& uAE w/ CU &  &  &  &  &  &  &  &  &  \\
\cline{2-11}
& iAE &  &  &  &  &  &  &  &  &  \\
& iAE w/ CU &  &  &  &  &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> Tables/exp_table_flat_unbiased.tex <==

\newcolumntype{?}{!{\vrule width 0.7pt}}

\begin{table*}[t]
\centering
\caption{Comparison results on Coat and Yahoo! R3 (* and ** indicate $p < 0.05$ and $p < 0.01$ for an one-tailed t-test). The suffix '-DU' indicates the existing model using dual unbiased learning (\eg, AT vs. AT-DU). The results are averaged over 10 and 5 runs on Coat and Yahoo! R3, respectively. \textit{Gain} indicates an improvement ratio to the corresponding unbiased model.}\label{tab:flat_unbiased}
\vspace{-3mm}
% $\dagger$ indicates baseline model for t-test and performance gain
\begin{center}
\renewcommand{\arraystretch}{1.2} % 테이블 행 간격
% \begin{tabular}{c c | c | c c : c | c c : c | c c : c}
\begin{tabular}{c c | c | c l | c | c l | c | c l | c}
% \begin{tabular}{c c | c | c l : c | c l : c | c l : c}
% \begin{tabular}{c c | c | c c c | c c c | c c c}
\toprule
Datasets & Metric & MF & Rel-MF & MF-DU & \textit{Gain (\%)} & AT & AT-DU & \textit{Gain (\%)} & CJMF & CJMF-DU & \textit{Gain (\%)} \\
\hline
\multirow{9}{*}{Coat}
& NDCG@1 & 0.3748 & 0.3959 & \textbf{0.4186}$^{**}$ & \com{\textit{+5.75}} & 0.4017 & \textbf{0.4345}$^{**}$ & \com{\textit{+8.15}} & 0.4093 & \textbf{0.4307}$^{*}$ & \com{\textit{+5.22}} \\
& NDCG@3 & 0.3441 & 0.3659 & \textbf{0.3718} & \com{\textit{+1.63}} & 0.3652 & \textbf{0.3748} & \com{\textit{+2.61}} & 0.3856 & \textbf{0.3984} & \com{\textit{+3.33}} \\
& NDCG@5 & 0.3714 & 0.3922 & \textbf{0.3984} & \com{\textit{+1.57}} & 0.3912 & \textbf{0.3965} & \com{\textit{+1.37}} & 0.4097 & \textbf{0.4256}$^{*}$ & \com{\textit{+3.87}} \\
\cline{2-12}
& MAP@1 & 0.1346 & 0.1484 & \textbf{0.1566}$^{*}$ & \com{\textit{+5.54}} & 0.1517 & \textbf{0.1609}$^{**}$ & \com{\textit{+6.07}} & 0.1500 & \textbf{0.1638}$^{**}$ & \com{\textit{+9.20}} \\
& MAP@3 & 0.2100 & 0.2281 & \textbf{0.2354} & \com{\textit{+3.20}} & 0.2286 & \textbf{0.2364}$^{*}$ & \com{\textit{+3.42}} & 0.2408 & \textbf{0.2524}$^{*}$ & \com{\textit{+4.83}} \\
& MAP@5 & 0.2566 & 0.2758 & \textbf{0.2821} & \com{\textit{+2.29}} & 0.2753 & \textbf{0.2817} & \com{\textit{+2.34}} & 0.2900 & \textbf{0.3067}$^{**}$ & \com{\textit{+5.75}} \\
\cline{2-12}
& Recall@1 & 0.1346 & 0.1484 & \textbf{0.1566}$^{*}$ & \com{\textit{+5.54}} & 0.1517 & \textbf{0.1609}$^{**}$ & \com{\textit{+6.07}} & 0.1500 & \textbf{0.1638}$^{**}$ & \com{\textit{+9.20}} \\
& Recall@3 & 0.2592 & 0.2819 & \textbf{0.2826} & \com{\textit{+0.27}} & 0.2772 & \textbf{0.2802} & \com{\textit{+1.10}} & 0.2984 & \textbf{0.3026} & \com{\textit{+1.41}} \\
& Recall@5 & 0.3705 & 0.3926 & \textbf{0.3952} & \com{\textit{+0.64}} & \textbf{0.3908} & 0.3820 & \rev{\textit{-2.26}} & 0.4075 & \textbf{0.4250}$^{*}$ & \com{\textit{+4.32}} \\
\hline
\multirow{9}{*}{Yahoo! R3}
& NDCG@1 & 0.1797 & 0.1837 & \textbf{0.2214}$^{**}$ & \com{\textit{+20.50}} & 0.1912 & \textbf{0.2209}$^{**}$ & \com{\textit{+15.52}} & 0.1810 & \textbf{0.2084}$^{**}$ & \com{\textit{+15.17}} \\
& NDCG@3 & 0.2081 & 0.2122 & \textbf{0.2469}$^{**}$ & \com{\textit{+16.37}} & 0.2179 & \textbf{0.2457}$^{**}$ & \com{\textit{+12.73}} & 0.2085 & \textbf{0.2374}$^{**}$ & \com{\textit{+13.90}} \\
& NDCG@5 & 0.2411 & 0.2453 & \textbf{0.2785}$^{**}$ & \com{\textit{+13.54}} & 0.2506 & \textbf{0.2783}$^{**}$ & \com{\textit{+11.07}} & 0.2404 & \textbf{0.2695}$^{**}$ & \com{\textit{+12.11}} \\
\cline{2-12}
& MAP@1 & 0.1071 & 0.1102 & \textbf{0.1373}$^{**}$ & \com{\textit{+24.56}} & 0.1149 & \textbf{0.1366}$^{**}$ & \com{\textit{+18.86}} & 0.1079 & \textbf{0.1269}$^{**}$ & \com{\textit{+17.63}} \\
& MAP@3 & 0.1688 & 0.1728 & \textbf{0.2068}$^{**}$ & \com{\textit{+19.68}} & 0.1786 & \textbf{0.2056}$^{**}$ & \com{\textit{+15.14}} & 0.1690 & \textbf{0.1964}$^{**}$ & \com{\textit{+16.18}} \\
& MAP@5 & 0.1970 & 0.2014 & \textbf{0.2364}$^{**}$ & \com{\textit{+17.40}} & 0.2071 & \textbf{0.2358}$^{**}$ & \com{\textit{+13.89}} & 0.1966 & \textbf{0.2255}$^{**}$ & \com{\textit{+14.70}} \\
\cline{2-12}
& Recall@1 & 0.1071 & 0.1102 & \textbf{0.1373}$^{**}$ & \com{\textit{+24.56}} & 0.1149 & \textbf{0.1366}$^{**}$ & \com{\textit{+18.86}} & 0.1079 & \textbf{0.1269}$^{**}$ & \com{\textit{+17.63}} \\
& Recall@3 & 0.2225 & 0.2266 & \textbf{0.2591}$^{**}$ & \com{\textit{+14.35}} & 0.2310 & \textbf{0.2575}$^{**}$ & \com{\textit{+11.48}} & 0.2220 & \textbf{0.2521}$^{**}$ & \com{\textit{+13.53}} \\
& Recall@5 & 0.3040 & 0.3080 & \textbf{0.3388}$^{**}$ & \com{\textit{+9.99}} & 0.3125 & \textbf{0.3395}$^{**}$ & \com{\textit{+8.62}} & 0.3016 & \textbf{0.3321}$^{**}$ & \com{\textit{+10.11}} \\
\bottomrule
\end{tabular}
\end{center}
% \vspace{1mm}
%\textit{Note}: The table reports the ranking metrics averaged over 10 different initializations for Coat and 5 for Yahoo! R3. \textit{Gain} = \(\frac{improvement}{baseline} * 100\).
\vspace{-3mm}
\end{table*}


==> Tables/exp_table_ml100k.tex <==
\begin{table*}[t]
\centering
\caption{Performance comparison of each model on ML100K benchmark dataset (the best in bold font).}\label{tab:ml100k}
\begin{center}
\begin{tabular}{P{1.5cm}P{1.5cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.0cm}}
\toprule

\multicolumn{2}{c}{} & \multicolumn{3}{c}{NDCG@K} & \multicolumn{3}{c}{MAP@K} & \multicolumn{3}{c}{Recall@K}\\
\cmidrule(r){3-5}
\cmidrule(lr){6-8}
\cmidrule(l){9-11}
 Evaluation & Models & K = 10 & K = 30 & K = 50 & K = 10 & K = 30 & K = 50 & K = 10 & K = 30 & K = 50  \\
\hline
\multirow{7}{*}{Unbiased}
& uAE       & 0.0195 & 0.0283 & 0.0329 & 0.0391 & 0.0521 & 0.0575 & 0.0867 & 0.1884 & 0.2571  \\
& iAE       & 0.0192 & 0.0280 & 0.0322 & 0.0386 & 0.0515 & 0.0568 & 0.0861 & 0.1856 & 0.2513  \\
& MF        & 0.0148 & 0.0231 & 0.0274 & 0.0293 & 0.0402 & 0.0448 & 0.0707 & 0.1628 & 0.2281  \\
\cline{2-11}
& Rel-MF    & 0.0204 & 0.0309 & 0.0364 & 0.0411 & 0.0563 & 0.0629 & 0.0985 & 0.2231 & 0.3083  \\
& AT        & 0.0210 & 0.0314 & 0.0374 & 0.0426 & 0.0584 & 0.0658 & 0.1013 & 0.2244 & 0.3168  \\
& CJMF      & 0.0211 & 0.0324 & 0.0382 & 0.0424 & 0.0591 & 0.0658 & 0.0974 & 0.2248 & 0.3126  \\
\cline{2-11}
& Proposed  & 0.0217 & 0.0328 & 0.0386 & 0.0436 & 0.0594 & 0.0659 & 0.0963 & 0.2210 & 0.3077  \\

% \hline
% \multirow{7}{*}{AOA}
% & uAE       & 0.2376 & 0.2710 & 0.3049 & 0.0943 & 0.1235 & 0.1352 & 0.1863 & 0.3449 & 0.4403  \\
% & iAE       & 0.2520 & 0.2876 & 0.3228 & 0.0996 & 0.1321 & 0.1449 & 0.1983 & 0.3688 & 0.4677  \\
% & MF        & 0.2535 & 0.2860 & 0.3203 & 0.1011 & 0.1319 & 0.1441 & 0.2003 & 0.3653 & 0.4614  \\
% \cline{2-11}
% & Rel-MF    & 0.2369 & 0.2867 & 0.3263 & 0.0987 & 0.1309 & 0.1438 & 0.1972 & 0.3881 & 0.4990  \\
% & AT        & 0.2535 & 0.3028 & 0.3414 & 0.1077 & 0.1419 & 0.1551 & 0.2047 & 0.4028 & 0.5113  \\
% & CJMF      & 0.2654 & 0.3160 & 0.3558 & 0.1106 & 0.1492 & 0.1638 & 0.2176 & 0.4221 & 0.5340  \\
% \cline{2-11}
% & Proposed  & 0.2857 & 0.3328 & 0.3744 & 0.1212 & 0.1616 & 0.1773 & 0.2306 & 0.4366 & 0.5546  \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> Tables/exp_table_pre-sipw_sipw.tex <==

\newcolumntype{?}{!{\vrule width 0.7pt}}

\begin{table}[t]
\centering
\caption{Accuracy comparison for the effect of self-inverse propensity weighting The results are averaged over 10 and 5 runs on Coat and Yahoo! R3, respectively. \textit{Gain} indicates an improvement ratio to the corresponding unbiased model.}\label{tab:flat_unbiased}
\vspace{-4mm}
% $\dagger$ indicates baseline model for t-test and performance gain
\begin{center}
\renewcommand{\arraystretch}{0.8} % 테이블 행 간격
\begin{tabular}{c c | c c | c}
\toprule
Datasets & Metric & MF & Rel-MF & \textit{Gain (\%)} \\
\hline
\multirow{9}{*}{Coat}
& NDCG@1 & 0.3748 & 0.3959 & \textbf{0.4186}$^{**}$ \\
& NDCG@3 & 0.3441 & 0.3659 & \textbf{0.3718} \\
& NDCG@5 & 0.3714 & 0.3922 & \textbf{0.3984} \\
\cline{2-12}
& MAP@1 & 0.1346 & 0.1484 & \textbf{0.1566}$^{*}$ \\
& MAP@3 & 0.2100 & 0.2281 & \textbf{0.2354} \\
& MAP@5 & 0.2566 & 0.2758 & \textbf{0.2821} \\
\cline{2-12}
& Recall@1 & 0.1346 & 0.1484 & \textbf{0.1566}$^{*}$ \\
& Recall@3 & 0.2592 & 0.2819 & \textbf{0.2826}\\
& Recall@5 & 0.3705 & 0.3926 & \textbf{0.3952} \\
\hline
\multirow{9}{*}{Yahoo! R3}
& NDCG@1 & 0.1797 & 0.1837 & \textbf{0.2214}$^{**}$ \\
& NDCG@3 & 0.2081 & 0.2122 & \textbf{0.2469}$^{**}$ \\
& NDCG@5 & 0.2411 & 0.2453 & \textbf{0.2785}$^{**}$ \\
\cline{2-12}
& MAP@1 & 0.1071 & 0.1102 & \textbf{0.1373}$^{**}$ \\
& MAP@3 & 0.1688 & 0.1728 & \textbf{0.2068}$^{**}$ \\
& MAP@5 & 0.1970 & 0.2014 & \textbf{0.2364}$^{**}$ \\
\cline{2-12}
& Recall@1 & 0.1071 & 0.1102 & \textbf{0.1373}$^{**}$ \\
& Recall@3 & 0.2225 & 0.2266 & \textbf{0.2591}$^{**}$ \\
& Recall@5 & 0.3040 & 0.3080 & \textbf{0.3388}$^{**}$ \\
\bottomrule
\end{tabular}
\end{center}
% \vspace{1mm}

\end{table}
s

==> Tables/exp_table_su_copy.tex <==
\begin{table}[t]
\centering
\caption{Accuracy comparison for the effect of self-inverse propensity weighting on Coat and Yahoo! R3 ($\dagger$ indicates the best baseline model for performance gain). The prefix `Rel' indicates adopting the IPW method of \citet{SaitoYNSN20}, and the suffix `+SIPW' indicates adopting the self-inverse propensity weighting. The results are averaged over 10 and 5 runs on Coat and Yahoo! R3, respectively. Gain indicates the improvement ratio from the best baseline model. Although we only report NDCG$@N$ results, we observe similar trends with the other metrics, MAP$@N$ and Recall$@N$.
}
% \vspace{-2mm}
\label{tab:su}
\begin{center}
\renewcommand{\arraystretch}{0.9} % 테이블 행 간격
\begin{tabular}{P{1.3cm}P{1.6cm}P{1.1cm}P{1.1cm}P{1.1cm}}
\toprule
 Datasets & Models & NDCG$@$1 & NDCG$@$3 & NDCG$@$5 \\
\hline
\multirow{12}{*}{Coat}
 & MF        & 0.3748          & 0.3441          & 0.3714          \\
 & RelMF$^{\dagger}$    & 0.3959          & 0.3659          & 0.3922          \\
 & MF + SIPW  & \textbf{0.3993} & \textbf{0.3686} & \textbf{0.3963} \\
 \cline{2-5}
 & Gain (\%) & 0.86            & 0.73            & 1.06            \\
 \cline{2-5}
 & UAE       & 0.3610          & 0.3546          & 0.3815          \\
 & RelUAE$^{\dagger}$   & 0.3876          & 0.3720          & 0.4031          \\
 & UAE + SIPW & \textbf{0.4262} & \textbf{0.3973} & \textbf{0.4259} \\
 \cline{2-5}
 & Gain (\%) & 9.96            & 6.79            & 5.65            \\
 \cline{2-5}
 & IAE       & 0.3655          & 0.3560          & 0.3812          \\
 & RelIAE$^{\dagger}$   & 0.3990          & 0.3716          & 0.3951          \\
 & IAE + SIPW & \textbf{0.4334} & \textbf{0.3949} & \textbf{0.4172} \\
 \cline{2-5}
 & Gain (\%) & 8.64            & 6.29            & 5.59            \\
\hline
\multirow{12}{*}{Yahoo! R3}
 & MF        & 0.1797          & 0.2081          & 0.2411          \\
 & RelMF$^{\dagger}$    & 0.1837          & 0.2122          & 0.2453          \\
 & MF + SIPW  & \textbf{0.1881} & \textbf{0.2176} & \textbf{0.2496} \\
 \cline{2-5}
 & Gain (\%) & 2.38            & 2.53            & 1.74            \\
 \cline{2-5}
 & UAE       & 0.1983          & 0.2235          & 0.2532          \\
 & RelUAE$^{\dagger}$   & 0.2054          & 0.2384          & 0.2715          \\
 & UAE + SIPW & \textbf{0.2115} & \textbf{0.2461} & \textbf{0.2785} \\
 \cline{2-5}
 & Gain (\%) & 2.96            & 3.25            & 2.54            \\
 \cline{2-5}
 & IAE       & 0.2137          & 0.2355          & 0.2653          \\
 & RelIAE$^{\dagger}$   & 0.2146          & 0.2398          & 0.2708          \\
 & IAE + SIPW & \textbf{0.2190} & \textbf{0.2504} & \textbf{0.2802} \\
 \cline{2-5}
 & Gain (\%) & 2.05            & 4.44            & 3.49            \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-2mm}
\end{table}


==> sec-fig.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{cc}
\includegraphics[height=3cm]{Figures/clicked_unclicked_cm100k_bar.png} $\;\;\;$
\includegraphics[height=3cm]{Figures/unclicked_cm100k_pie.png.png} \\
\end{tabular}
\vspace{-2mm}
\caption{Statistics on different rating types (\ie, relevance and observation) in CM100K. The left figure shows the distribution of clicked and unclicked data. The right figure represents the ratio of three cases of unclicked data.}\label{fig:cm100k}
\vspace{-2mm}
\end{figure}


%Left is distribution of clicked and unclicked data. Right is the proportion of three cases of unclicked data. CM100K has observation and relevance for all ratings.
%; CM100K has observation and relevance information for all ratings



==> sec-model__backup_.tex <==
\section{Proposed Framework}
\label{sec:model}

% \subsection{Motivation}
% \label{sec:motivation}
In this section, we first investigate the bias of model predictions by conventional recommender models, \ie, matrix factorization (MF) and autoencoders (AE)~\cite{SedhainMSX15} on the MovieLens-100K (ML-100K) dataset. Figures~\ref{fig:motive_fig}(a) and (c) depict a positive correlation between the average predicted scores for clicked items and the number of ratings, \ie, popularity, in the training set. Because the conventional models are biased by the popularity of items in the training set, popular items tend to be recommended to more users. As a result, the biased recommendation can exacerbate the bias of the training dataset as user feedback is continually collected.


To address this problem, it is vital to eliminate the bias of observed user feedback. Existing studies~\cite{Saito20, SaitoYNSN20} mainly focused on modeling the popularity bias. In contrast, because the user experiences are mostly biased by the recommended items, we aim at eliminating the exposure bias by recommender models. That is, we estimate the propensity score for the exposure bias and remove it during model training. Figures~\ref{fig:motive_fig}(b) and (d) show our unbiased learning method, removing the exposure bias of items. It is clearly observed that the correlation between the rating distribution and the predicted values is weaker than the traditional models in Figures~\ref{fig:motive_fig}(a) and (c), indicating that our proposed estimation effectively reduces the exposure bias.



\subsection{The BISER Framework}
\label{sec:overview}


In this section, we overview a novel unbiased recommender framework, namely \emph{Bilateral Self-unbiased Recommender (BISER)}. Specifically, it consists of two parts: \emph{self-inverse propensity weighting} and \emph{bilateral unbiased learning}, as depicted in Figure~\ref{fig:proposed}. Inspired by self-distillation~\cite{MobahiFB20,YangXSY19} that iteratively extracts knowledge of model predictions during model training, we first introduce inverse propensity weighting (IPW) in an iterative manner. Our proposed weighting is beneficial because it requires neither a pre-defined propensity scoring function nor an additional model for propensity estimation. Also, we train two recommender models with complementary characteristics to mitigate the high variance of propensity scores. Although it is model-agnostic, we adopt user- and item-based autoencoders, capturing different user- and item-side hidden patterns from an entire dataset. As a result, we can bypass conformity bias, which occurs when the outputs of multiple models converge similarly in training with the same training sets.

\vspace{1mm}
\noindent
\textbf{Surrogate-guided inverse propensity weighting.} We employ inverse propensity weighting (IPW), commonly used in the literature~\cite{SaitoYNSN20,Saito20,ZhuHZC20}. The core part of designing IPW is to estimate the propensity score indicating the click bias. For that, existing studies deal with the click bias in two directions: 1) by modeling the popularity bias of items, which affects the user behavior of clicking items regardless of the mechanism of recommender models~\cite{SaitoYNSN20,Saito20,ZhuHZC20}, or 2) by adopting an additional model to estimate the exposure bias by interleaving relevance and observation estimation~\cite{ZhuHZC20}. However, they only focus on predicting the exposure bias on the collected data and do not take into account the bias of the recommender model.

To deal with this issue, we design a new bias estimation method with a surrogate model, namely \emph{surrogate-guided inverse propensity weighting (SIPW)}. For that, we first analyze a biased recommender model using click data. Given a model with parameters $\theta$, the probability of clicking an item in Eq.~\eqref{eq:click} is given by

\begin{equation}
  \label{eq:click_proposed}
  P(y_{ui} = 1 | \theta) = P(o_{ui} = 1 | \theta) \cdot P(r_{ui} = 1 | \theta).
\end{equation}

Under this setting, the probability of clicking an item $i$ by a user $u$ is explicitly affected by its exposure probability by the recommender model. Notably, as the true relevance of an item to a user is independent of the recommender model, we can set $P(r_{ui} = 1 | \theta) = P(r_{ui} = 1)$. Inspired by \cite{WangBMN16}, we can estimate the inverse propensity score $\omega_{ui}$ in Eq.~\eqref{eq:saito} with the prediction of uniformly trained model by

\begin{equation}
  \label{eq:click_proposed}
  \frac{P(y_{ui} = 1 | \theta)}{P(y_{ui} = 1 | \theta')} \propto P(o_{ui} = 1 | \theta) = \hat{\omega}_{ui},
\end{equation}

\noindent
where $\theta'$ is uniformpy trained surrogate model of $\theta$. (We will state how we train the $\theta'$. formally state our loss function in Section~\ref{sec:learning}.)

Finally, we can formally devise an unbiased loss function using surrogate-guided inverse propensity weighting:
\begin{equation}
\label{eq:self_unbiased}
  \mathcal{L}_{SIPW}(\hat{\textbf{R}}; \theta) = \frac{1}{|\mathcal{D}|}\sum_{(u, i) \in \mathcal{D}}{ \left(\frac{y_{ui}}{\hat{\omega}_{ui}} \delta^{+}_{ui} + \left ( 1-\frac{y_{ui}}{\hat{\omega}_{ui}} \right )\delta^{-}_{ui} \right)}.
\end{equation}
As $\hat{\omega}_{ui}$ continues to change during training. That is, we make the model prediction for $y_{ui}$, and then iteratively utilize it for $\hat{\omega}_{ui}$ as model training continues.

Although it is simple, our proposed estimation can effectively eliminate the bias of the recommender model, as depicted in Figures~\ref{fig:motive_fig}(b) and (d). 

% Secondly, because it is model-agnostic, we can apply various recommender models, \eg, MF~\cite{HuKV08} and AE~\cite{SedhainMSX15}.




% \vspace{1mm}
% \noindent
% \textbf{Self-inverse propensity weighting.} We employ inverse propensity weighting (IPW), commonly used in the literature~\cite{SaitoYNSN20,Saito20,ZhuHZC20}. The core part of designing IPW is to estimate the propensity score indicating the click bias. For that, existing studies deal with the click bias in two directions: 1) by modeling the popularity bias of items, which affects the user behavior of clicking items regardless of the mechanism of recommender models~\cite{SaitoYNSN20,Saito20,ZhuHZC20}, or 2) by adopting an additional model to estimate the exposure bias by interleaving relevance and observation estimation~\cite{ZhuHZC20}. Because the bias estimation model is trained with the relevance model, it considers the selection bias imposed by recommender systems. However, \citet{ZhuHZC20} splits an entire dataset into multiple training and estimation subsets, as done in cross-validation evaluation, incurring too much computational overhead. 


% In this paper, we design a new bias estimation method without an additional model, namely \emph{self-inverse propensity weighting (SIPW)}. For that, we first analyze a biased recommender model using click data. Given a model with parameters $\theta$, the probability of clicking an item in Eq.~\eqref{eq:click} is given by
% \begin{equation}
%   \label{eq:click_proposed}
%   P(y_{ui} = 1 | \theta) = P(o_{ui} = 1 | \theta) \cdot P(r_{ui} = 1 | \theta).
% \end{equation}

% Under this setting, the probability of clicking an item $i$ by a user $u$ is explicitly affected by its exposure probability by the recommender model. Notably, as the true relevance of an item to a user is independent of the recommender model, we can set $P(r_{ui} = 1 | \theta) = P(r_{ui} = 1)$. Based on this property, we can estimate the inverse propensity score $\omega_{ui}$ in Eq.~\eqref{eq:saito} using the model prediction by
% \begin{equation}
% \label{eq:click_propen_relation}
%   \hat{\omega}_{ui} = \frac{P(y_{ui} = 1 | \theta)}{P(r_{ui} = 1 | \theta)} = \frac{P(y_{ui} = 1 | \theta)}{P(r_{ui} = 1)} = \alpha P(y_{ui} = 1 | \theta),
% \end{equation}
% where $\alpha = \frac{1}{P(r_{ui} = 1)}$ is the inverse relevance of an item $i$ to a user $u$. That is, the exposure probability of an item is proportional to its model prediction. This is intuitive because the model learns the distribution of labels. It is empirically observed in Figures~\ref{fig:motive_fig}(a) and (c). For the clicked item, we empirically set $\alpha = 1$.

% %because the click contains a positive preference (relevance).
% % For the unclicked item, we assume that the $\alpha$ is constant because the preference is ambiguous.



% % It means that as an item is more frequently recommended, the item is regarded as a more biased one.

% %This indicates that the recommender model can iteratively restrict the probability of exposing items to the user. That is, the user is more likely to click items provided by the recommender, and this promotes those popular items even more, and so on. 


% Based on $\hat{\omega}_{ui}$ in Eq.~\eqref{eq:click_propen_relation}, we formally devise an unbiased loss function using self-inverse propensity weighting:
% \begin{equation}
% \label{eq:self_unbiased}
%   \mathcal{L}_{SIPW}(\hat{\textbf{R}}; \theta) = \frac{1}{|\mathcal{D}|}\sum_{(u, i) \in \mathcal{D}}{ \left(\frac{y_{ui}}{\hat{\omega}_{ui}} \delta^{+}_{ui} + \left ( 1-\frac{y_{ui}}{\hat{\omega}_{ui}} \right )\delta^{-}_{ui} \right)}.
% \end{equation}
% As $\hat{\omega}_{ui}$ continues to change during training. (We will formally state our loss function in Section~\ref{sec:learning}.) That is, we make the model prediction for $y_{ui}$, and then iteratively utilize it for $\hat{\omega}_{ui}$ as model training continues.

% Although it is simple, our proposed estimation has several benefits. Firstly, we can effectively eliminate the bias of click data, as depicted in Figures~\ref{fig:motive_fig}(b) and (d). Secondly, because it is model-agnostic, we can apply various recommender models, \eg, MF~\cite{HuKV08} and AE~\cite{SedhainMSX15}. Lastly, we can efficiently compute propensity scores without requiring additional model training.





\vspace{1mm}
\noindent
\textbf{Bilateral unbiased learning.} Although the IPW is theoretically principled, it often leads to sub-optimal performance due to the high variance problem in practice~\cite{SwaminathanJ15,GilotteCNAD18,WangZSQ19}. Existing study~\cite{Saito20at} utilized training multiple models, where predictions from one model are used as pseudo-labels for the other models. Then, the pseudo-label is used to regularize the model. Although it helps to mitigate the high variance problem, using multiple models may incur another issue called \emph{conformity bias}. That is, multiple models show similar tendencies as they get trained.

To resolve this issue, we introduce two models with complementary characteristics. In conventional recommender models, it is known that unifying user- and item-based recommender models lead to improve predictions~\cite{WangVR06,YamashitaKS11,ZhuWC19}. Since they capture different user and item patterns, adopting user- and item-based models can bypass the conformity bias and reinforce the advantages of two models in mutual model training.


Specifically, we utilize user- and item-based autoencoders to learn non-linear and complex user-item interactions. Inspired by label shift~\cite{LiptonWS18, Azizzadenesheli19}, \ie, the distribution of the features is the same even if the distribution of the labels is different, we assume that the true user preference (item relevance) is independent of model's label predictions. Formally,
\begin{equation}
  \label{eq:assumption2}
  P(r_{ui} = 1 | y_{ui} = 1, \theta_U) = P(r_{ui} = 1 | y_{ui} = 1, \theta_I),
\end{equation}
where $\theta_U$ and $\theta_I$ are the parameters for the user- and item-based autoencoders~\cite{SedhainMSX15}.

Finally, we design the loss function for bilateral unbiased learning using these two models:
\begin{equation}
  \label{eq:co_unbiased}
  \mathcal{L}_{BU}(\hat{\textbf{R}}; \theta_U, \theta_I) = \frac{1}{|\tilde{\mathcal{D}}|}\sum_{(u, i) \in \tilde{\mathcal{D}}}{ \left( \hat{y}_{ui | \theta_U} - \hat{y}_{ui | \theta_I}\right)^2},
\end{equation}
where $\hat{y}_{ui | \theta_U}$ and $\hat{y}_{ui | \theta_I}$ are predictions from each model. Also, $\tilde{\mathcal{D}}$ is a set of clicked user-item pairs.




\subsection{Training and Inference}
\label{sec:learning}
\noindent
Given user- and item-based autoencoders, each model is trained from scratch with self-inverse propensity weighting. At each epoch, we update the model parameters by minimizing the loss below:


\begin{equation}
  \label{eq:self_unbiased_epoch}
  \mathcal{L}_{SIPW}(\hat{\textbf{R}}; \theta^{(k)}) = \frac{1}{|\mathcal{D}|}\sum_{(u, i) \in \mathcal{D}}{ \left(\frac{y_{ui}}{\hat{\omega}_{ui | \theta^{(k)}}} \delta^{+}_{ui} + \left ( 1-\frac{y_{ui}}{\hat{\omega}_{ui | \theta^{(k)}}} \right )\delta^{-}_{ui} \right)},
\end{equation}
where $\theta^{(k)}$ indicates the model parameters at the $k$-th epoch and $\hat{\omega}_{ui | \theta^{(k)}}$ is self-inverse propensity score for $y_{ui}$ at the $k$-th epoch.

Next, we formulate the loss function to regularize the model parameter $\theta^{(k)}$ by minimizing the difference between two model predictions for each epoch. In other words, the model with parameter $\theta^{(k)}$ is trained with the prediction of another model with parameter $\psi^{(k)}$ as pseudo-labels, in order to reduce the variance of model predictions:
\begin{equation}
\label{eq:co_unbiased_epoch}
  \mathcal{L}_{BU}(\hat{\textbf{R}}; \theta^{(k)}, \psi^{(k)}) = \frac{1}{|\tilde{\mathcal{D}}|}\sum_{(u, i) \in \tilde{\mathcal{D}}}{ \left( \hat{y}_{ui | \theta^{(k)}} - \hat{y}_{ui | \psi^{(k)}}\right)^2}.
\end{equation}


Using the two loss functions in Eq.~\eqref{eq:self_unbiased_epoch} and~\eqref{eq:co_unbiased_epoch}, we can represent the final loss function in training each model at the $k$-th epoch:
\begin{align}
  \label{eq:proposed_final_1}
  \mathcal{L}_\text{UAE}(\hat{\textbf{R}}; \theta_U^{(k)}) & = \mathcal{L}_{SIPW}(\hat{\textbf{R}}; \theta_U^{(k)}) + \lambda_U\mathcal{L}_{BU}(\hat{\textbf{R}}; \theta_U^{(k)}, \theta_I^{(k)}), \\
  \label{eq:proposed_final_2}
  \mathcal{L}_\text{IAE}(\hat{\textbf{R}}; \theta_I^{(k)}) & = \mathcal{L}_{SIPW}(\hat{\textbf{R}}; \theta_I^{(k)}) + \lambda_I\mathcal{L}_{BU}(\hat{\textbf{R}}; \theta_I^{(k)}, \theta_U^{(k)}),
\end{align}
where $\lambda_U$ and $\lambda_I$ are the hyper-parameters to control relative importance of $\mathcal{L}_{BU}$. 

% Empirically, we set $\lambda_U = 0.01$ and $\lambda_I = 0.01$.



\input{learning_algo}


Algorithm~\ref{alg:algorithm1} describes the pseudo-code of our proposed model with user- and item-based autoencoders. In the learning process, it first initializes parameters $\theta_U$ and $\theta_I$ of both autoencoders (line 1). At each epoch, it first calculates both models' predictions for all clicked user-item pairs, using the parameters from the previous epoch (line 3). Then, $\theta_U$ and $\theta_I$ are updated using Eq.~\eqref{eq:proposed_final_1} and Eq.~\eqref{eq:proposed_final_2}, respectively (line 5 and 8).


After model training, we have unbiased user- and item-based autoencoders. The biases of these two models are eliminated from the user's point of view and the item's point of view, respectively. By unifying preferences from different perspectives, our proposed model enjoys improved predictions~\cite{WangVR06,YamashitaKS11,ZhuWC19}. For the final prediction, we take the average of the predicted preferences of the two models:
\begin{equation}
  \label{eq:inferofBISEL}
  \hat{y}_{ui} = \frac{\hat{y}_{ui | \theta_U} + \hat{y}_{ui | \theta_I}}{2}.
\end{equation}

% \vspace{0.2cm}

==> sec-relatedwork_cikm_ver.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Unbiased Learning-to-Rank (LTR)}

Unbiased learning has been widely used for causal inference~\cite{WangBMN16, JoachimsSS17, WangGBMN18, AiBLGC18, HuWPL19, Wang0WW21, OvaisiAZVZ20, SchnabelSSCJ16, 0003ZS021, WangZSQ19, Saito20at, SaitoYNSN20, Saito20, ZhuHZC20, QinCMNQW20} and missing data analysis~\cite{MarlinZRS07, Steck10, HernHG14, MarlinZ09, abs-1808-06581, MaC19, LiangCMB16}. Then, it has been adopted for bridging the gap between click data and relevant data in the information retrieval (IR) community, \ie, unbiased learning-to-rank (LTR). To formulate unbiased LTR, existing studies consider several types of bias, \ie, position bias and selection bias. 


\vspace{1mm}
\noindent
\textbf{Eliminating position bias.} The position bias means that the user tends to click the top-ranked documents. To eliminate position bias, existing studies~\cite{JoachimsSS17, WangGBMN18, AiBLGC18, HuWPL19, Wang0WW21} mostly estimate the propensity scores depending on the position of documents. \citet{JoachimsSS17} calculated the propensity score using the randomization method. It randomly shuffles the position of relevant documents and then uses the click-through rate of each position as the propensity score. To overcome randomization that hurts the user experience, \citet{WangGBMN18} estimated the propensity score with the regression-based EM method. Also, \citet{AiBLGC18} jointly trained the propensity model and ranker to get the propensity score estimator. \citet{HuWPL19} extended the point-wise based jointly learning method to the pair-wise based method. Unlike previous studies that only considered bias in click data, \citet{Wang0WW21} estimated the propensity score for both clicked and unclicked data to remove the bias for unclicked feedback as well.


\vspace{1mm}
\noindent
\textbf{Eliminating selection bias.} The selection bias indicates that the user tends to click the documents on the first page of ranking results provided by the search engine. To eliminate selection bias, \citet{WangBMN16} assumed that the selection bias was equal to the position bias of the ranking result generated by the ranker. Then, they removed the bias by the randomization method. Also, \citet{OvaisiAZVZ20} used Heckman's two-stage method to remove the selection bias. It first classifies whether the document is on the first page of search results and then removes the position bias with the propensity model.


\subsection{Unbiased Recommender Learning}

Inspired by unbiased LTR, unbiased recommender learning has been actively studied to eliminate bias from user feedback.

\vspace{1mm}
\noindent
\textbf{Unbiased learning with explicit feedback.} Although explicit feedback provides positive and negative preferences, it is also based on the MNAR assumption. Specifically, users tend to rate more of some items they think are relevant, \ie, self-selection bias. To address this problem, existing studies can be categorized into three directions: \emph{imputation-based}, \emph{IPW-based}, and \emph{meta-learning-based methods}. Firstly, imputation-based methods~\cite{MarlinZRS07, Steck10, HernHG14, MarlinZ09, abs-1808-06581, MaC19} estimates some ratings for missing feedback to reduce biased statistics of user ratings. \citet{Steck10} imputed a predefined constant value to all missing feedback. Then, some studies utilize various recommender models to impute different ratings; \citet{HernHG14, abs-1808-06581} used an MF model, \citet{MarlinZRS07} used a multinomial mixture model, and \citet{MarlinZ09} used a conditional Bernoulli model. Recently, \citet{MaC19} adopted nuclear-norm-constrained matrix completion algorithm~\cite{abs-1209-3672} for rating imputation. Secondly, IPW-based methods~\cite{SchnabelSSCJ16, 0003ZS021, WangZSQ19} are used to estimate propensity scores for user-item ratings. \citet{SchnabelSSCJ16} first adopted the IPW method and predicted the propensity score using Naïve Bayes or logistic regression, and \citet{0003ZS021} trained a propensity estimator with few unbiased ratings. Also, \citet{WangZSQ19} combined the IPW and the imputation method to eliminate bias to take advantage of both methods. Recently, the meta-learning-based method~\cite{Saito20at} was adopted to overcome the high variance problem of IPW. This method used multiple models instead of IPW method to train a model without variance. Specifically, \citet{Saito20at} trained a model using the output of one of several models as unbiased pseudo-labels. The main difference between the above related methods and the proposed method is that the purpose of the related method is rating prediction well, but the purpose of the proposed method is \topN~ recommendation well by removing the bias.

\vspace{1mm}
\noindent
\textbf{Unbiased learning with implicit feedback.} Unlike explicit feedback, implicit feedback only provides clicked and unclicked user feedback. Therefore, it is essential to design the exposure bias for items. Specifically, the exposure bias can be considered from user- and model-oriented reasons. Because users tend to recognize popular items, user click is biased to popular items as well, \ie, popularity bias. To eliminate the popularity bias, \citet{LiangCMB16} determined the weight based on the prior probability of exposure. Also, \cite{SaitoYNSN20, Saito20, ZhuHZC20} use the IPW-based method to remove the bias. While \cite{SaitoYNSN20, Saito20} simply utilized the number of ratings per item (\ie, item's popularity) as the propensity score, \cite{ZhuHZC20} used an additional model to estimate a propensity score. Recently, \citet{QinCMNQW20} also introduced a propensity estimator that used additional attributes related to the recommender model (\eg, UI of application, type of recommender model), which can consider the exposure bias by recommender models. In clear contrast, our proposed method focuses on removing exposure bias by recommender model without additional information as well model training.

